BMTree: Designing, Learning, and Updating Piecewise Space-Filling Curves for Multi-Dimensional Data Indexing

Space-filling curves (SFC, for short) have been widely applied to index multi-dimensional data, which first maps the data to one dimension, and then a one-dimensional indexing method, e.g., the B-tree indexes the mapped data. Existing SFCs adopt a single mapping scheme for the whole data space. However, a single mapping scheme often does not perform well on all the data space. In this paper, we propose a new type of SFC called piecewise SFCs that adopts different mapping schemes for different data subspaces. Specifically, we propose a data structure termed the Bit Merging tree (BMTree) that can generate data subspaces and their SFCs simultaneously, and achieve desirable properties of the SFC for the whole data space. Furthermore, we develop a reinforcement learning-based solution to build the BMTree, aiming to achieve excellent query performance. To update the BMTree efficiently when the distributions of data and/or queries change, we develop a new mechanism that achieves fast detection of distribution shifts in data and queries, and enables partial retraining of the BMTree. The retraining mechanism achieves performance enhancement efficiently since it avoids retraining the BMTree from scratch. Extensive experiments show the effectiveness and efficiency of the BMTree with the proposed learning-based methods.

==> sections/discussion.tex <==
\revision{
%\subsection{Discussion}

\noindent {\bf Handling updates.} 
% \marginpar{\#3 W1}
{\jn In the presence of insertion,
%or deletion, 
%the indexes combined with 
the BMTree can still be  applied as the mapping function to compute SFC values for new data points.
%, and maintain the index structure. 
In the experiment, we observe that the query performance on indexes built on the SFC values from the BMTree is 
%relatively 
insensitive to moderate shifts in data and query distribution. 
%, resulting in minimal performance degradation when the BMTree remains unchanged.
However, in the case of a sharp change in query distribution, a  retraining of the BMTree is recommended to maintain %optimal 
its performance.}

% In our experiment, we observe that BMTree is relatively insensitive to shifts in data distribution but is sensitive to changes in query distribution. 
% Therefore, during insertion/deletion, whether it follows the former data distribution or not, the index can directly apply the current BMTree as the mapping function to maintain the index structure with minimal performance degradation. However, the BMTree needs to be retrained when query workload has a sharp change in distribution.

% While BMTree can tolerate data insertion or deletion, a sharp change in query distribution requires retraining and building a new index based on the updated BMTree.

% In experiment, we evaluated the effect when data or query distribution is shifting. The result shows that BMTree is less sensitive to data distribution shifting, while is sensitive to query. Therefore, BMTree can tolerate the data insertion or deletion. However, when query distribution suffers a sharp change, it is preferable to retrain the BMTree with the new query workload. And then new index can be built based on the new BMTree.

\iffalse
\noindent {\bf Optimizing other queries.} This paper 
%primarily 
focuses on optimizing window queries. 
%However, there are also other types of queries such as $k$NN query. 
However, other queries, e.g., $k$NN queries, can also be included in the optimization objective as part of the workload. We will empirically evaluate if window queries and $k$NN queries can be %jointly 
optimized together. 
%The results indicate the potential of our method with a mixed objective.
% In the evaluation section, we designs experiment to see (1) how the optimization of window query effect $k$NN query performance, (2) and evaluate if our method can trade off between different queries with a mixed objective.


}
\fi
